Mining on Manifolds: Metric Learning without Labels

In this work we present a novel unsupervised framework for hard training example mining. The only input to the method is a collection of images relevant to the target application and a meaningful initial representation, provided e.g. by pre-trained CNN. Positive examples are distant points on a single manifold, while negative examples are nearby points on different manifolds. Both types of examples are revealed by disagreements between Euclidean and manifold similarities. The discovered examples can be used in training with any discriminative loss. The method is applied to unsupervised fine-tuning of pre-trained networks for fine-grained classification and particular object retrieval. Our models are on par or are outperforming prior models that are fully or partially supervised.

==> ext-plots.tex <==
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{pgf,tikz}

\usepackage{tikzextern}
%\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{figs/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> intro.tex <==
\section{Introduction}
\label{sec:intro}

The success of deep learning is \emph{de facto} connected to supervised classification: this is the task where convolutional networks were first demonstrated~\cite{KSH12}, feature learning was shown superior to hand-crafted visual features~\cite{LBD+90}, and most network architectures are pre-trained before being used for other tasks~\cite{SZ14,SLJS+15,HZRS16}. There are tasks that require predicting a progressively finer level of visual similarity, including fine-grained classification~\cite{WCMD16}, particular object retrieval~\cite{GARL16}, local descriptor learning~\cite{HLJ+15}, ranking~\cite{WSL+14}, and nearest-neighbor regression~\cite{BSSO16}. Metric learning~\cite{CHL05,WSL+14,HKC+17} is more suitable for such tasks, being based on relations between more than one samples at a time.

However, most recent deep metric learning approaches still use class labels to define such relations in the first place. This is unsatisfying not only because we miss the opportunity of learning from unlabeled data, but learned representations of each class are inevitably unimodal. Attempted remedies are \emph{post-hoc} and typically based on some form of clustering~\cite{RPDB15,MeHD17,BaSO17}. Therefore, while investigating loss functions alternative to cross-entropy (\eg contrastive~\cite{HaCL06}, triplet~\cite{WSL+14} or batch-level~\cite{OXJS16}) and data sampling for efficiency~\cite{HKC+17,MTL+17}, the nature of the problem essentially remains the same as supervised classification.

%------------------------------------------------------------------
\begin{figure}
\small
\begin{center}
\includegraphics[height=1.7cm]{fig/intro/banana_euclidean.pdf}\hspace{6pt}
\includegraphics[height=1.7cm]{fig/intro/banana_manifold.pdf}\\
\hspace{5pt}(a) Euclidean NN (orange) \hspace{20pt} (b) Manifold NN (purple)\\ \vspace{1pt}
\includegraphics[height=1.7cm]{fig/intro/banana_pos.pdf}\hspace{6pt}
\includegraphics[height=1.7cm]{fig/intro/banana_neg.pdf}\\
\hspace{5pt}(c) Hard positives (green) \hspace{20pt} (d) Hard negatives (red)
\end{center}
\vspace{-1pt}
\caption{Given an anchor point (black) and its $k$ nearest Euclidean (\nne{k}) and manifold (\nnd{k}) neighbors in a dataset, we choose positive samples as $\nnd{k} \setminus \nne{k}$, and negative as $\nne{k} \setminus \nnd{k}$. Data is unlabeled and the selection is fully unsupervised, including anchors.
\vspace{-1pt}
\label{fig:intro}
}
\end{figure}
%------------------------------------------------------------------

Because similarities in the original input space are not trusted, most unsupervised methods seek proxy supervision in the underlying data, by devising new tasks or by automating the annotation process. For instance, exploiting the temporal dimension in video~\cite{WG15,1708.02901}, predicting the spatial layout of image patches~\cite{Doersch_2017_ICCV}, or using existing computer vision pipelines to match unstructured image collections pairwise~\cite{GARL16,RTC16}. This approach does change the nature of the problem and requires no or little human effort, but makes assumptions on the data or requires a domain-specific oracle. It is also sensitive to label noise.

Conventional nonlinear dimension reduction or manifold learning methods do trust the nearest neighbor relations in the input space, as well as approximate geodesic distances computed from the former~\cite{TSL00,SR03,BN03}. However, most do not learn an explicit mapping from the input to the embedding space. Hence, handling new samples is awkward and expensive. On the other hand, recent metric learning methods do learn powerful mappings, but rarely use the underlying manifold structure in the data. We attempt to bridge this gap in this work.

Our idea is very simple and is illustrated in Figure~\ref{fig:intro}. We start from any representation space of unlabeled data and assume there is an efficient way to measure manifold distances or similarities in that space. Given a anchor point that is part of the data, neighbors on the manifold that are not Euclidean neighbors are considered positive samples, in the sense that if we are to learn a new representation space, they should be attracted to the anchor. Conversely, Euclidean neighbors that are not neighbors on the manifold are considered negative and should be repelled.

Essentially, this is a hard positive or negative mining process with the `similar/dissimilar' labels determined by the underlying manifold. Hence any discriminative loss applies like contrastive or triplet. The manifold similarity is estimated by a random walk on the nearest neighbor graph of the original representation, which is an efficient alternative to a geodesic distance. Anchors are chosen by mode seeking, again following a random model.

Our learning process is entirely unsupervised. We make no assumptions \eg on spatial or temporal relations and use no models other than the one we are optimizing. Our input is just unlabeled data and our output is an explicit mapping to a new representation space for measuring fine similarities that generalizes well to new data. We apply to fine-grained classification and to particular object retrieval by unsupervised fine-tuning of pre-trained networks. Our models are on par or are outperforming prior models that are supervised in one way or another.

The paper is organized as follows. Section~\ref{sec:related} discusses related work. Sections~\ref{sec:method}\ref{sec:applications} present our learning method and applications, respectively. Experiments are given in Section~\ref{sec:experiments} conclusions are drawn in Section~\ref{sec:conclusions}.



==> no-plots.tex <==
\newcommand{\extfig}[2]{!}
\newcommand{\extdata}[1]{}


==> tab_allSel.tex <==
% \begin{center}
% \small
% \begin{tabular}{ |@{\msp}l@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|}
%     \hline
%                               & CUB-200-2011    & Oxf5k - Rand 		& Oxf5k - GM     		\\ \hline  \hline
%       Baseline                & 42.2        	& 52.6          	& 52.6					\\ 
%       kNN                     & 44.2        	& 37.4          	& 64.4					\\ 
%       Graph-Pos               & 45.5        	& 48.2          	& 38.1					\\ 
%       Graph-Neg               & 45.8       		& 57.8          	& 71.3					\\ 
%       Graph-Full              & 46.1        	& 64.4          	& 73.7					\\ 
%       Graph-Full + W          & \textbf{47.1}   & 67.0          	& \textbf{76.7}			\\ \hline 

% \end{tabular}

\begin{center}
\small
\begin{tabular}{ |@{\msp}l@{\msp}|@{\msp}c@{\msp}|c|@{\msp}c@{\msp}|@{\msp}c@{\msp}|}
    \hline
      \multirow{2}{*}{Positives}  							& \multirow{2}{*}{Negatives}  	& CUB-200-2011    	& \multicolumn{2}{c|}{Oxford5k}      		\\ 
      				  										&								& all				& random			& $\cA$ 				\\ \hline \hline
      \multicolumn{2}{|@{\nsp}c@{\nsp}|}{Baseline}											& 35.0        		& 52.6          	& 52.6										\\ 
      \nne{5}                    							& $\setminus$\nne{5}			& 38.5        		& 37.4          	& 64.4					\\ 
      $\cP^+$               								& $\setminus$\nne{5}			& 43.0        		& 48.2          	& 38.1					\\ 
      \nne{5}               								& $\cP^- $						& 42.1       		& 57.8          	& 71.3					\\ 
      $\cP^+$              									& $\cP^- $						& 43.5        		& 64.4          	& 73.7					\\ 
      $\cP^+ + w$          									& $\cP^- + w$					& \textbf{45.3}   	& 67.0          	& \textbf{76.7}			\\ \hline 

\end{tabular}


==> tab_cubsoa.tex <==
\begin{center}
\small
\begin{tabular}{ |@{\msp}l@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|}
    \hline
                        							&	Labels		& R@1     & R@2		& R@4		& R@8		& NMI		\\ \hline  \hline
      Baseline          							& \checkmark	& 35.0    & 46.8  	& 59.3  	& 72.0  	& 48.1  	\\ 
      Triplet-sh~\cite{SKP15}*  					& \checkmark	& 42.8	  & 55.9  	& 68.2  	& 79.6  	& 54.7  	\\ 
      LS~\cite{OXJS16}*  							& \checkmark	& 44.8    & 58.3  	& 70.5  	& 80.3		& 56.4    	\\
      Triplet~\cite{HKC+17}  						& \checkmark	& 45.9    & 57.7  	& 69.6  	& 79.8		& 58.1    	\\ 
      Clustering~\cite{SJRM17}  					& \checkmark	& 48.2    & 61.4  	& 71.8  	& 81.9		& 59.2    	\\ 
      Tr + GA\cite{HKC+17}  						& \checkmark	& 49.8    & 62.3  	& 74.1  	& 83.3		& 59.9    	\\ \hline  \hline

      Ours              							& \xmark		& 45.3    & 57.8    & 68.6   	& 78.4    	& 55.0   	\\ \hline

\end{tabular}


==> tab_retrsoa.tex <==
% \begin{center}
% \begin{tabular}{ |@{\msp}l@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|}
%     \hline
%                         							&			& Oxford5k		& Oxford105k 	& Paris6k			& Paris106k		& Holidays			& Instre			\\ \hline  \hline
%       \multirow{2}{*}{Baseline~\cite{TSJ15}}     	& MAC		& 58.5			& 50.3			& 73.0  			& 59.0			& 79.4  			& 48.5  			\\ \cline{2-8}
%            					 						& R-MAC		& 68.0	  		& 61.0	  		& 76.6  			& 72.1  		& 87.0  			& 55.6  			\\ \hline
%       \multirow{2}{*}{siaMAC~\cite{RTC16}}			& MAC		& \textbf{79.7}	& 73.9    		& 82.4  			& 74.6  		& 81.4				& 48.5    			\\ \cline{2-8}
%         											& R-MAC		& 77.8			& 70.1    		& 84.1    			& 76.8   		& 84.4    			& 47.7   			\\ \hline
%       \multirow{2}{*}{Ours}       					& MAC		& 78.7			& \textbf{74.3} & 83.1  			& 75.6  		& 82.6				& 55.5    			\\ \cline{2-8}
%          											& R-MAC		& 78.2			& 72.6    		& \textbf{85.1}  	& \textbf{78.0} & \textbf{87.5}    	& \textbf{57.7}   	\\ \hline
% \end{tabular}


\begin{center}
\begin{tabular}{ |@{\msp}l@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|@{\msp}c@{\msp}|}
    \hline
                        							&							& Oxford5k		& Oxford105k 	& Paris6k			& Paris106k		& Holidays			& Instre			\\ \hline  \hline
      Baseline~\cite{TSJ15}     					& \multirow{3}{*}{MAC}		& 58.5			& 50.3			& 73.0  			& 59.0			& 79.4  			& 48.5  			\\ \cline{2-8}
      siaMAC~\cite{RTC16}							& 							& \textbf{79.7}	& 73.9    		& 82.4  			& 74.6  		& 81.4				& 48.5    			\\ \cline{2-8}
      Ours       									& 							& 78.7			& \textbf{74.3} & 83.1  			& 75.6  		& 82.6				& 55.5    			\\ \cline{2-8}
      Baseline~\cite{TSJ15} 						& \multirow{3}{*}{R-MAC}	& 68.0	  		& 61.0	  		& 76.6  			& 72.1  		& 87.0  			& 55.6  			\\ \hline
      siaMAC~\cite{RTC16}							& 							& 77.8			& 70.1    		& 84.1    			& 76.8   		& 84.4    			& 47.7   			\\ \hline
      Ours											& 							& 78.2			& 72.6    		& \textbf{85.1}  	& \textbf{78.0} & \textbf{87.5}    	& \textbf{57.7}   	\\ \hline
\end{tabular}

